Model-based Subsampling for Knowledge Graph Completion

Subsampling is effective in Knowledge Graph Embedding (KGE) for reducing overfitting caused by the sparsity in Knowledge Graph (KG) datasets. However, current subsampling approaches consider only frequencies of queries that consist of entities and their relations. Thus, the existing subsampling potentially underestimates the appearance probabilities of infrequent queries even if the frequencies of their entities or relations are high. To address this problem, we propose Model-based Subsampling (MBS) and Mixed Subsampling (MIX) to estimate their appearance probabilities through predictions of KGE models. Evaluation results on datasets FB15k-237, WN18RR, and YAGO3-10 showed that our proposed subsampling methods actually improved the KG completion performances for popular KGE models, RotatE, TransE, HAKE, ComplEx, and DistMult.

==> results_short.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\resizebox{0.95\columnwidth}{!}{
\small
\begin{tabular}{lllllll}
\toprule
\multicolumn{7}{c}{\textbf{FB15k-237}}                               \\\midrule
\textbf{Model} & \multicolumn{2}{c}{\textbf{Subsampling}} & \textbf{MRR} & \textbf{Hits@1} & \textbf{Hits@3} & \textbf{Hits10}\\\midrule
\multirow{13}{*}{RotatE}        & \multicolumn{2}{c}{None} & 32.9 & 22.9 & 37.0 & 53.1 \\
\cmidrule{2-7} & \multirow{3}{*}{Base} &  CBS & 33.7 & 23.9 & \textbf{37.6} & 53.3 \\\cmidrule{3-7}
                                && MBS & 33.9 & 24.1 & 37.5 & \textbf{53.5} \\
                                && MIX & \textbf{34.0} & \textbf{24.3} & \textbf{37.6} & 53.4  \\\cmidrule{2-7}
                                & \multirow{3}{*}{Freq}  & CBS  & 34.1 & 24.7  & 37.6 & 53.2 \\\cmidrule{3-7}
                                && MBS & 34.3 & 24.7 & 38.0 & \textbf{53.6} \\
                                && MIX & \textbf{34.6}$^{\dagger}$ & \textbf{25.1} & \textbf{38.1} & \textbf{53.6} \\\cmidrule{2-7}
                                & \multirow{3}{*}{Uniq} & CBS & 34.0 & 24.6 & 37.5 & 53.0 \\\cmidrule{3-7}
                                && MBS & 34.3 & 24.8 & 37.9 & 53.6          \\
                                && MIX & \textbf{34.6}$^{\dagger}$ & \textbf{25.2}$^{\dagger}$ & \textbf{38.4}$^{\dagger}$ & \textbf{53.7}$^{\dagger}$ \\\midrule
\multirow{13}{*}{ComplEx}       &\multicolumn{2}{c}{None} & 22.3 & 13.9 & 24.1 & 39.5 \\
\cmidrule{2-7}& \multirow{3}{*}{Base} &  CBS & 32.2 & 22.9 & 35.4 & 51.2 \\\cmidrule{3-7}
                                && MBS & 31.3 & 21.3 & 34.8 & 51.7 \\
                                && MIX & \textbf{32.5} & \textbf{23.0} & \textbf{35.8} & \textbf{52.3}$^{\dagger}$ \\
                                \cmidrule{2-7}& \multirow{3}{*}{Freq}  & CBS & 32.7  & 23.4 & 36.0 & 51.2 \\\cmidrule{3-7}
                                && MBS & 31.8 & 22.7 & 34.9 & 49.9          \\
                                && MIX & \textbf{32.8}$^{\dagger}$ & \textbf{23.6}$^{\dagger}$ & \textbf{36.2}$^{\dagger}$ & \textbf{51.4} \\\cmidrule{2-7}
                                & \multirow{3}{*}{Uniq} & CBS  & \textbf{32.6}  & \textbf{23.4}  & \textbf{35.8} & 51.0 \\\cmidrule{3-7}
                                & & MBS & 31.9    & 22.7  & 34.9  & 50.6          \\
                                & & MIX & \textbf{32.6}   & \textbf{23.4} & 35.6 & \textbf{51.2} \\\midrule
\multirow{13}{*}{HAKE}&         \multicolumn{2}{c}{None} & 32.4 & 22.0 & 36.9 & 53.1 \\
\cmidrule{2-7} & \multirow{3}{*}{Base}  & CBS  & \textbf{34.6}   & \textbf{24.8}  & 38.4  & 54.1  \\\cmidrule{3-7}
                                &  & MBS & 34.4  & 24.5 & 38.0  & \textbf{54.2} \\
                                & & MIX & 34.5   & 24.7 & \textbf{38.5} & \textbf{54.2} \\\cmidrule{2-7}
                                & \multirow{3}{*}{Freq} & CBS  & 35.2  & 25.7 & 38.7 & \textbf{54.5} \\\cmidrule{3-7}
                                &  & MBS  & \textbf{35.3} & \textbf{25.8}  & \textbf{39.1} & 54.4          \\
                                &  & MIX & \textbf{35.3}  & 25.7 & 39.0   & \textbf{54.5} \\\cmidrule{2-7}
                                & \multirow{3}{*}{Uniq} & CBS  & 35.2 & 25.6  & 38.7   & 54.6 \\\cmidrule{3-7}
                                & & MBS  & 35.3  & 25.6 & \textbf{39.2}$^{\dagger}$ & \textbf{54.7}$^{\dagger}$ \\
                                & & MIX & \textbf{35.4}$^{\dagger}$   & \textbf{25.9}$^{\dagger}$   & 39.0  & 54.6   \\\bottomrule
\end{tabular}}
\caption{Results on FB15k-237. The bold scores are the best results for each subsampling type (e.g. Base, Freq, and Uniq.). $\dagger$ indicates the best scores for each model.\label{tab:fb15k-237}}
\end{table}

\begin{table}[t]
\centering
\resizebox{0.95\columnwidth}{!}{
\small
\begin{tabular}{lllllll}
\toprule
\multicolumn{7}{c}{\textbf{WN18RR}}\\\midrule
\textbf{Model} & \multicolumn{2}{c}{\textbf{Subsampling}} & \textbf{MRR} & \textbf{Hits@1} & \textbf{Hits@3} & \textbf{Hits10}\\\midrule
\multirow{13}{*}{RotatE}&                \multicolumn{2}{c}{None}  & 47.3 & 42.9 & 48.8 & 55.7 \\
\cmidrule{2-7}         & \multirow{3}{*}{Base}  & CBS   & 47.9 & \textbf{43.7}  & 49.5  & 55.7   \\\cmidrule{3-7}
                                & & MBS & \textbf{48.0}  & 43.4 & \textbf{49.8}$^{\dagger}$ & \textbf{57.4}$^{\dagger}$ \\
                                &   & MIX   & 47.9   & 43.4    & 49.7    & 56.7   \\\cmidrule{2-7}
                                & \multirow{3}{*}{Freq}  & CBS   & 47.9   & 43.2   & 49.6   & 56.8   \\\cmidrule{3-7}
                                &  & MBS  & \textbf{48.0}   & \textbf{43.3} & \textbf{49.8}$^{\dagger}$ & \textbf{57.0} \\
                                & & MIX   & 47.9  & \textbf{43.3} & 49.5  & 56.9  \\\cmidrule{2-7}
                                & \multirow{3}{*}{Uniq}  & CBS  & 47.9    & 43.1 & 49.7  & \textbf{57.3} \\\cmidrule{3-7}
                                & & MBS  & 48.0 & 43.6  & 49.6  & 56.8     \\
                                & & MIX   & \textbf{48.2}$^{\dagger}$  & \textbf{43.8}$^{\dagger}$   & \textbf{49.8}$^{\dagger}$ & 56.8   \\\midrule
\multirow{13}{*}{ComplEx}&      \multicolumn{2}{c}{None}   & 45.0 & 40.9 & 46.6 & 53.5 \\
\cmidrule{2-7}   & \multirow{3}{*}{Base}   & CBS  & 46.8   & 42.4 & 48.5  & \textbf{55.6} \\\cmidrule{3-7}
                                && MBS   & 47.2  & \textbf{43.3}  & 48.8 & 54.7     \\
                                &  & MIX   & \textbf{47.3}     & 43.2  & \textbf{49.0} & 55.3   \\\cmidrule{2-7}
                                & \multirow{3}{*}{Freq}  & CBS  & 47.2   & 42.7  & 49.3  & 56.2   \\\cmidrule{3-7}
                                & & MBS  & \textbf{48.6}$^{\dagger}$   & \textbf{44.5}$^{\dagger}$  & \textbf{50.4}$^{\dagger}$ & 56.8   \\
                                & & MIX  & \textbf{48.6}$^{\dagger}$   & \textbf{44.5}$^{\dagger}$ & 50.3   & \textbf{57.0}$^{\dagger}$ \\\cmidrule{2-7}
                                & \multirow{3}{*}{Uniq}  & CBS  & 47.5 & 43.1 & 49.0  & 56.2 \\\cmidrule{3-7}
                                &  & MBS  & 48.3   & 44.2 & \textbf{49.9} & \textbf{56.5} \\
                                &  & MIX  & \textbf{48.4}  & \textbf{44.4} & \textbf{49.9} & 56.4   \\\midrule
\multirow{13}{*}{HAKE}&         \multicolumn{2}{c}{None}  & 49.0 & 44.6 & 50.7 & 57.5 \\
\cmidrule{2-7}   & \multirow{3}{*}{Base}      & CBS    & \textbf{49.5}  & \textbf{45.1}   & \textbf{51.3} & 58.0  \\\cmidrule{3-7}
                                &   & MBS   & 49.1  & 44.5  & \textbf{51.3} & 57.9          \\
                                &   & MIX  & 49.4    & 44.9 & \textbf{51.3} & \textbf{58.4} \\\cmidrule{2-7}
                                & \multirow{3}{*}{Freq} & CBS & \textbf{50.0}   & \textbf{45.5}    & 51.9 & 58.2   \\\cmidrule{3-7}
                                & & MBS   & 49.9   & 45.3 & \textbf{52.0}$^{\dagger}$ & \textbf{58.3} \\
                                & & MIX  & 49.8 & 45.4 & 51.6    & 58.1  \\\cmidrule{2-7}
                                & \multirow{3}{*}{Uniq} & CBS  & 49.7  & 45.2  & 51.5  & 58.2   \\\cmidrule{3-7}
                                &   & MBS   & \textbf{50.1}$^{\dagger}$   & \textbf{45.6}$^{\dagger}$ & \textbf{51.8} & \textbf{58.5}$^{\dagger}$ \\
                                &  & MIX  & 50.0    & \textbf{45.6}$^{\dagger}$ & 51.7   & \textbf{58.5}$^{\dagger}$\\
\bottomrule
\end{tabular}}
\caption{Results on WN18RR. The notations are the same as the ones in Table \ref{tab:fb15k-237}.\label{tab:wn18rr}}
\end{table}

==> selected.tex <==
\begin{table}[t]
    \centering
    \resizebox{\columnwidth}{!}{
    \small
    \begin{tabular}{|l|c|ll|ll|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Subsampling}} & \multicolumn{4}{c|}{\textbf{Sub-model}} \\
    \cline{3-6}
    && \multicolumn{2}{c|}{\textbf{FB15k-237}} & \multicolumn{2}{c|}{\textbf{WN18RR}} \\
    \hline
    \multirow{3}{*}{RotatE} & Base & ComplEx & None & ComplEx & None \\
    & Freq & ComplEx & None & ComplEx & None \\
    & Uniq & ComplEx & None & ComplEx & None \\
    \hline
    \multirow{3}{*}{ComplEx} & Base & ComplEx & None & ComplEx & None \\
    & Freq & ComplEx & Base & ComplEx & None \\
    & Uniq & ComplEx & Base & ComplEx & None \\
    \hline
    \multirow{3}{*}{HAKE} & Base & ComplEx & None & ComplEx & None \\
    & Freq & ComplEx & Base & ComplEx & None \\
    & Uniq & RotatE & Base & ComplEx & None \\
    \hline
    \end{tabular}}
    \caption{Selected sub-models for MBS based on the validation MRR on FB15k-237 and WN18RR.}
    \label{tab:selected}
\end{table}


==> settings.tex <==
\begin{table}[h!]
% \begin{sidewaystable}
    % \vspace{1cm}
    \centering
    %\resizebox{0.6\textwidth}{!}{
    \small
    \begin{tabular}{|l|c|llll|llll|}
    \hline
    \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Subsampling}} & \multicolumn{8}{c|}{\textbf{Sub-model}} \\
    \cline{3-10}
    && \multicolumn{4}{c|}{\textbf{FB15k-237}} & \multicolumn{4}{c|}{\textbf{WN18RR}} \\
    \hline
    \multirow{3}{*}{RotatE} & Base & ComplEx & None & $\alpha$: 0.5 & $\lambda$: 0.9 & ComplEx & None & $\alpha$: 1.0 & $\lambda$: 0.5 \\
    & Freq & ComplEx & None & $\alpha$: 0.1 & $\lambda$: 0.7 & ComplEx & None & $\alpha$: 0.5 & $\lambda$: 0.3 \\
    & Uniq & ComplEx & None & $\alpha$: 0.1 & $\lambda$: 0.5 & ComplEx & None & $\alpha$: 0.5 & $\lambda$: 0.5 \\
    \hline
    \multirow{3}{*}{ComplEx} & Base & ComplEx & None & $\alpha$: 1.0 & $\lambda$: 0.5 & ComplEx & None & $\alpha$: 2.0 & $\lambda$: 0.7 \\
    & Freq & ComplEx & Base & $\alpha$: 0.5  & $\lambda$: 0.1 & ComplEx & None & $\alpha$: 0.5 & $\lambda$: 0.9 \\
    & Uniq & ComplEx & Base & $\alpha$: 0.5 &$\lambda$: 0.1 & ComplEx & None & $\alpha$: 0.5 & $\lambda$: 0.9 \\
    \hline
    \multirow{3}{*}{HAKE} & Base & ComplEx & None & $\alpha$: 1.0 & $\lambda$: 0.5 & ComplEx & None & $\alpha$: 1.0 & $\lambda$: 0.3 \\
    & Freq & ComplEx & Base & $\alpha$: 0.5 & $\lambda$: 0.5 & ComplEx & None & $\alpha$: 1.0 & $\lambda$: 0.1 \\
    & Uniq & RotatE & Base & $\alpha$: 0.5 & $\lambda$: 0.3 & ComplEx & None & $\alpha$: 0.5 & $\lambda$: 0.7 \\
    \hline
    \end{tabular}
    %}
    \caption{Selected sub-models and other settings based on the validation MRR.}
    \label{tab:settings}
% \end{sidewaystable}
\end{table}
